Combination of inclusive top-quark pair production cross-section measurements using ATLAS and CMS data at $\sqrt{s}= 7$ and 8 TeV

A combination of measurements of the inclusive top-quark pair production cross-section performed by ATLAS and CMS in proton-proton collisions at centre-of-mass energies of 7 and 8 TeV at the LHC is presented. The cross-sections are obtained using top-quark pair decays with an opposite-charge electron-muon pair in the final state and with data corresponding to an integrated luminosity of about 5 fb$^{-1}$ at $\sqrt{s}=7$ TeV and about 20 fb$^{-1}$ at $\sqrt{s}=8$ TeV for each experiment. The combined cross-sections are determined to be $178.5 \pm 4.7$ pb at $\sqrt{s}=7$ TeV and $243.3^{+6.0}_{-5.9}$ pb at $\sqrt{s}=8$ TeV with a correlation of 0.41, using a reference top-quark mass value of 172.5 GeV. The ratio of the combined cross-sections is determined to be $R_{8/7}= 1.363\pm 0.032$. The combined measured cross-sections and their ratio agree well with theory calculations using several parton distribution function (PDF) sets. The values of the top-quark pole mass (with the strong coupling fixed at 0.118) and the strong coupling (with the top-quark pole mass fixed at 172.5 GeV) are extracted from the combined results by fitting a next-to-next-to-leading-order plus next-to-next-to-leading-log QCD prediction to the measurements. Using a version of the NNPDF3.1 PDF set containing no top-quark measurements, the results obtained are $m_t^\text{pole} = 173.4^{+1.8}_{-2.0}$ GeV and $\alpha_\text{s}(m_Z)= 0.1170^{+ 0.0021}_{-0.0018}$.

==> packages_and_commands.tex <==
\RequirePackage{hepnames}
	
\RequirePackage{longtable}

\newcommand{\cmsAuthorMark}[1]{\hbox{\textsuperscript{\normalfont#1}}}
\newcommand{\cmsinstitute}[1]{\par\pagebreak[3]\bfseries #1 \mdseries\\[0pt]}
\newcommand{\cmsorcid}[1]{\href{https://orcid.org/#1}{\hspace*{0.1em}\raisebox{-0.45ex}{\includegraphics[width=1em]{ORCIDiD_iconvector.pdf}}}}



%define in lhcphysics
%\renewcommand{\TeV}{\ensuremath{\,\text{Te\hspace{-.08em}V}}\xspace}
%\renewcommand{\TeV}{\ensuremath{~\text{Te\hspace{-.08em}V}}\xspace}
%define in lhcphysics
%\renewcommand{\GeV}{\ensuremath{\,\text{Ge\hspace{-.08em}V}}\xspace}
%\renewcommand{\GeV}{\ensuremath{~\text{Ge\hspace{-.08em}V}}\xspace}
%\newcommand{\fbinv} {\mbox{\ensuremath{\,\text{fb}^\text{$-$1}}}\xspace}
\newcommand{\fbinv} {\mbox{\ensuremath{~\text{fb}^\text{$-$1}}}\xspace}

%define in lhcphysics
%\newcommand{\pt}{\ensuremath{p_{\mathrm{T}}}\xspace}
%define in lhcphysics
%\newcommand{\ttbar}    {\ensuremath{\Ptop \APtop}\xspace}
\newcommand{\xsec}    {\ensuremath{\sigma_{\Ptop \APtop}}\xspace}
\newcommand{\mtpole}{\ensuremath{m_t^{\text{pole}}}\xspace}
\newcommand{\mt}{\ensuremath{m_t}\xspace}


\newcommand{\emu}{\ensuremath{e\mu}\xspace}
\newcommand{\W}{\ensuremath{W}\xspace}
\newcommand{\bq}{\ensuremath{b}\xspace}

%\newcommand{\toppp}{Top++\xspace}
\newcommand{\toppp}{\textsc{Top++}\xspace}         % DPS: ATLAS style

%ATLAS variables
\newcommand{\epsem}{\mbox{$\epsilon_{e\mu}$}}
\newcommand{\cb}{\mbox{$C_b$}}
\newcommand{\nib}{\mbox{$N_1^{\rm bkg}$}}
\newcommand{\niib}{\mbox{$N_2^{\rm bkg}$}}
\newcommand{\epsb}{\mbox{$\epsilon_{b}$}}
\newcommand{\intlumiATLa}{4.6}
\newcommand{\intlumiATLb}{20.2}
\newcommand{\xtt}{\ensuremath{\sigma_{\ttbar}}\xspace}
\newcommand{\sxv}{\mbox{$\sqrt{s}=8$\,\TeV}}
\newcommand{\sxw}{\mbox{$\sqrt{s}=7$\,\TeV}}
\newcommand{\sxvt}{$\sqrt{s}=8$\,\TeV}
\newcommand{\sxwt}{$\sqrt{s}=7$\,\TeV}
% measured quantities for 2011
\newcommand{\ttxvalw}{182.9}
\newcommand{\ttxstatw}{3.1}
\newcommand{\ttxsystw}{4.2}
\newcommand{\ttxlumiw}{3.6}
\newcommand{\ttxebeamw}{3.3}
\newcommand{\ttxtotw}{7.1}
\newcommand{\ttxrelw}{3.9\,\%}
\newcommand{\ttxrelsystw}{2.3\,\%}
\newcommand{\intlumiw}{4.6}
\newcommand{\wcutw}{0.601713}
% meausred quantities for 2012, updated with new luminosity uncertainty from 20/3/16
\newcommand{\ttxval}{242.9}
\newcommand{\ttxstat}{1.7}
\newcommand{\ttxsyst}{5.5}
\newcommand{\ttxlumi}{5.1}
\newcommand{\ttxebeam}{4.2}
\newcommand{\ttxtot}{8.8}
\newcommand{\ttxrel}{3.6\,\%}
\newcommand{\ttxrelsyst}{2.3\,\%}


% Combination Results: updated Apr 3
% 7 TeV
\newcommand{\ttxvalcombs}{178.5}
\newcommand{\ttxtotpcombs}{4.7}
\newcommand{\ttxtotmcombs}{4.7}
\newcommand{\ttxrelcombs}{2.7\,\%}
% 8 TeV
\newcommand{\ttxvalcombe}{243.3}
\newcommand{\ttxtotpcombe}{6.0}
\newcommand{\ttxtotmcombe}{5.9}
\newcommand{\ttxrelcombe}{2.5\,\%}
\newcommand{\rhocomb}{0.41}
% Ratio
\newcommand{\ttxratio}{1.363}
\newcommand{\ttxratioerr}{0.032}
\newcommand{\ttxratiostaterr} {0.015}
\newcommand{\ttxratiosysterr} {0.028}
 

% Mass and alphas results: 
%CT14: updated May 13th
\newcommand{\massCT}{174.0}
\newcommand{\massuncCTup}{{2.3}}
\newcommand{\massuncCTdown}{{2.3}}
\newcommand{\massuncrelCT}{1.3\,\%}
\newcommand{\alphasCT}{0.1161}
\newcommand{\alphasuncCTup}{{0.0030}}
\newcommand{\alphasuncCTdown}{{0.0033}}
\newcommand{\alphasuncrelCT}{2.8\,\%}
%MMHT2014: updated May 13th
\newcommand{\massMMHT}{174.0}
\newcommand{\massuncMMHTup}{{2.1}}
\newcommand{\massuncMMHTdown}{{2.3}}
\newcommand{\massuncrelMMHT}{1.3\,\%}
\newcommand{\alphasMMHT}{0.1160}
\newcommand{\alphasuncMMHTup}{{0.0031}}
\newcommand{\alphasuncMMHTdown}{{0.0030}}
\newcommand{\alphasuncrelMMHT}{2.7\,\%}

%NNPDF30: updated April 6th
\newcommand{\massNN}{173.70}
\newcommand{\massuncNN}{1.92}
\newcommand{\massuncrelNN}{1.10\,\%}
\newcommand{\alphasNN}{0.1156}
\newcommand{\alphasuncNN}{0.0038}
\newcommand{\alphasuncrelNN}{3.31\,\%}

%NNPDF31 ascorrnotop: updated May 13th
\newcommand{\massNNascorrnotop}{173.4}
\newcommand{\massuncNNascorrnotopup}{{1.8}}
\newcommand{\massuncNNascorrnotopdown}{{2.0}}
%\newcommand{\massuncrelNNascorrnotop}{1.2\,\%}
\newcommand{\massuncrelNNascorrnotop}{1.2\%}                % DPS: space removed
\newcommand{\alphasNNascorrnotop}{0.1170}
\newcommand{\alphasuncNNascorrnotopup}{{0.0021}}
\newcommand{\alphasuncNNascorrnotopdown}{{0.0018}}
%\newcommand{\alphasuncrelNNascorrnotop}{1.8\,\%}
\newcommand{\alphasuncrelNNascorrnotop}{1.8\%}               % DPS: space removed

%NNPDF31 nominal: updated April 6th
\newcommand{\massNNnom}{172.81}
\newcommand{\massuncNNnom}{1.80}
\newcommand{\massuncrelNNnom}{1.04\,\%}
\newcommand{\alphasNNnom}{0.1172}
\newcommand{\alphasuncNNnom}{0.0029}
\newcommand{\alphasuncrelNNnom}{2.49\,\%}



